PencilNet: Zero-Shot Sim-to-Real Transfer Learning for Robust Gate Perception in Autonomous Drone Racing

In autonomous and mobile robotics, one of the main challenges is the robust on-the-fly perception of the environment, which is often unknown and dynamic, like in autonomous drone racing. In this work, we propose a novel deep neural network-based perception method for racing gate detection -- PencilNet -- which relies on a lightweight neural network backbone on top of a pencil filter. This approach unifies predictions of the gates' 2D position, distance, and orientation in a single pose tuple. We show that our method is effective for zero-shot sim-to-real transfer learning that does not need any real-world training samples. Moreover, our framework is highly robust to illumination changes commonly seen under rapid flight compared to state-of-art methods. A thorough set of experiments demonstrates the effectiveness of this approach in multiple challenging scenarios, where the drone completes various tracks under different lighting conditions.

==> large_elements/fig_simulation_pipeline.tex <==
\tikzstyle{int}=[draw, align=center, fill=blue!0, minimum size=2em, text width=.75cm]
\begin{tikzpicture}[node distance=1cm,auto,>=latex]
    \node[int, line width=0.5mm, text width=2cm, minimum height=1cm, fill=yellow!25] (ue) {Unreal Engine};
    \node[int, line width=0.5mm, above = 0.5 of ue, text width=2cm, minimum height=1cm, fill=blue!25] (pose) {Random Gate Pose};
    \node[inner sep=0, below = 0.5 of ue, label=below:Gate mesh] (mesh) {\includegraphics[width=2.5cm]{figures/pipeline_mesh.png}};
    \node[inner sep=0, right = 0.5 of ue, label=above:Wide-angle image] (scene) {\includegraphics[width=2.5cm]{figures/pipeline_scene.png}};
    \node[inner sep=0, right = 0.5 of scene, label=above:Fish-eye image] (fisheye) {\includegraphics[width=2.5cm]{figures/pipeline_fisheye.png}};
    \node[inner sep=0, below = 0.5 of fisheye, label=below:Pencil-filter image] (pencil) {\includegraphics[width=2.5cm]{figures/pipeline_pencil.png}};
                   
    \draw[->, line width=0.5mm] (pose.south) -- (ue.north);
    \draw[->, line width=0.5mm] (mesh.north) -- (ue.south);
    \draw[->, line width=0.5mm] (ue.east) -- (scene.west);
    \draw[->, line width=0.5mm] (scene.east) -- (fisheye.west);
    \draw[->, line width=0.5mm] (fisheye.south) -- (pencil.north);
\end{tikzpicture}
